Geometric Contact Potential

Barrier potentials gained popularity as a means for robust contact handling in physical modeling and for modeling self-avoiding shapes. The key to the success of these approaches is adherence to geometric constraints, i.e., avoiding intersections, which are the cause of most robustness problems in complex deformation simulation with contact. However, existing barrier-potential methods may lead to spurious forces and imperfect satisfaction of the geometric constraints. They may have strong resolution dependence, requiring careful adaptation of the potential parameters to the object discretizations. We present a systematic derivation of a continuum potential defined for smooth and piecewise smooth surfaces, starting from identifying a set of natural requirements for contact potentials, including the barrier property, locality, differentiable dependence on shape, and absence of forces in rest configurations. Our potential is formulated independently of surface discretization and addresses the shortcomings of existing potential-based methods while retaining their advantages. We present a discretization of our potential that is a drop-in replacement for the potential used in the Incremental Potential Contact (IPC) formulation, and compare its behavior to other potential formulations, demonstrating that it has the expected behavior. The presented formulation connects existing barrier approaches, as all recent existing methods can be viewed as a variation of the presented potential, and lays a foundation for developing alternative (e.g., higher-order) versions.

==> 04-teaser.tex <==
\begin{teaserfigure}
    \centering
    \includegraphics[width=\linewidth]{figs/teaser.pdf}
    \caption{
     
     We introduce a novel geometric barrier potential satisfying a set of natural properties. None of the other potentials in the literature satisfy all these properties simultaneously, leading to inaccurate results, penetrations, or other undesired artifacts. In this example, we show that the contact potential introduced in \cite{Li2020IPC} is not zero at the rest pose (top) when the potential extent is larger than the length of an edge, introducing spurious forces. Our potential is zero in the rest pose by construction (bottom), as this is one of the natural properties of a geometric contact potential.}    
    \label{fig:teaser}
\end{teaserfigure}


==> 10-introduction.tex <==
\section{Introduction}
\label{sec:intro}



Contact modeling is a critical component of simulation tools for many domains, including physical simulation for computer graphics, robotics,  mechanical design, and biomedical engineering.  Recent advances, in particular, \ac{IPC}~\cite{Li2020IPC}, have made it possible to perform, in a reliable way, complex, large-deformation, and long-duration simulations of deformable objects with self-contact, with minimal parameter tuning.  

The fundamental principle of IPC solvers is strict adherence to geometric constraints over the entire trajectory (no intersections including self-intersections), even when approximations are made in other aspects of the problem.  This feature is the key to robustness. Overwhelmingly, robustness issues in contact mechanics are geometric in nature; once a contact constraint is violated, it may be very difficult for the simulation to recover. 

Geometric constraint satisfaction in IPC is accomplished by a combination of using a geometric barrier function, i.e. an interaction potential that approaches infinity as the simulation configuration approaches contact, and conservative \ac{CCD}. The IPC formulation excels at its main goal, qualitatively improving the robustness of contact simulations. 

The fundamental limitation of the IPC potential is that it was designed directly for discretized models, rather than obtained from a discretization of a continuum potential, as we discuss in more detail in \cref{sec:related}.   The purely discrete nature of IPC makes its behavior under remeshing and refinement hard to analyze and control, compared, e.g., to standard FEM discretizations of elasticity. It also precludes further developments such as adaptivity based on error estimation and improving accuracy by increasing discretization order.  Even more significantly, the dependence of the potential parameters on discretization leads to \emph{unavoidable} strong artificial forces in certain configurations.

\begin{wrapfigure}{L}{0.15\textwidth}
    \includegraphics[clip,width=0.15\textwidth]{figs/sketches/nearby-points.pdf}
    \caption{Contact potentials must distinguish points nearing contact (A and B) from nearby non-contacting points (A and C).}
    \label{fig:nearby-points}
\end{wrapfigure}

An essential property of a contact barrier potential used in deformable simulation with self-contact, which we will define precisely in  Section~\ref{sec:requirements}, is that the potential, on the one hand, guarantees that no interpenetration can occur (i.e., the potential becomes infinite if there is contact), and at the same time, does not cause spurious repulsion between nearby points on the object. In other words, 
the potential needs to distinguish true contact, arising from different objects or parts of the surface of the same object moving toward each other, and points that remain close because these are close on the undeformed rest shape (\cref{fig:nearby-points}). For smooth surfaces, points in true contact have opposing normals. IPC formulation and its version described in \cite{Li2023Convergent}, do not always distinguish these correctly, leading to 
strong artificial forces (see Section~\ref{sec:spurious-eval}). 
 

In this paper, we undertake a systematic derivation of a \emph{continuum barrier potential} defined as a surface integral and its discretization, which retains key features of IPC, but distinguishes between true contact and close material points,  and satisfies several natural requirements,  
which we make more precise in \cref{sec:requirements}:

\begin{itemize} 
    \item \Rindep:  The potential definition is independent of discretization. 
    \item \Rgen: The total barrier potential over the surface is defined and finite for any collection of piecewise-smooth surfaces not in contact. (The use of piecewise-smooth, rather than smooth, surfaces is critical for many applications.) 
    \item \Rbar: The potential grows to infinity as the objects in the simulation approach (self-)contact,  with respect to a suitably defined \emph{distance-to-contact}. 
    \item \Rloc: The potential has a localization parameter $\hat{d}$, which may vary over the object surface, but is fixed in time. The potential vanishes if the objects are further away than $\hat{d}$ from contact, with respect to the same measure of contact.
    \item \Rrest: In the undeformed configuration, the potential is zero.
    \item \Rdiff: The potential depends smoothly on the surface configuration (e.g., for piecewise-linear surfaces, on mesh vertex positions).
\end{itemize}

Three requirements (\Rbar, \Rloc, and \Rrest) depend on choosing a measure of distance to contact. How we measure this distance for self-contact is critical for defining the potential (\cref{sec:requirements}).   For IPC, the implied distance to contact is discretization-dependent: if we define it as the distance between closest vertices, \Rbar and \Rloc are satisfied, but not \Rindep, or \Rrest, leading to severe force artifacts whenever this distance is below $\hat{d}$, even in the absence of true contact, e.g., as a consequence of compression, thin membranes, or refining the discretization.

The foundation of our approach is a \emph{new geometric definition of the distance-to-contact} that allows us to define contact potentials for arbitrary piecewise-smooth surfaces without assuming a discretization, and in a way that all requirements are satisfied, leading to artifact-free simulation with a flexible choice of potential locality.  The key features of our approach include: 



\begin{itemize} 
\item  The concept of \emph{{\interaction} sets}, that, in turn, supports a definition of our distance-to-contact. 
\item  An approach for defining a contact potential for piecewise-smooth surfaces 
that meets the requirements enumerated above. 
\item A discrete version of this potential for piecewise-linear surfaces that satisfies the requirements enumerated above and has similar efficiency to standard IPC.
\end{itemize}

We demonstrate in a set of experiments that our formulation avoids spurious, discretization-dependent forces introduced by the original IPC formulation \cite{Li2020IPC} (\cref{sec:eval}) while retaining its main features and efficiency. The decoupling of the locality from mesh resolution further reduces the parameter tuning required for scenes with large deformations (\cref{sec:eval}).


==> 20-related.tex <==
\section{Barrier potentials}
\label{sec:related-barrier}

To motivate the proposed approach, we consider several versions of contact potentials proposed in the past. 

We focus on four problems that each construction addresses differently: 
\begin{itemize}
\item \emph{Finiteness.} How the potentials ensure that true contact points are distinguished from close material points; without this distinction, they would always be infinite.  
\item \emph{Spurious repulsion.} Relatedly, how spurious forces for close material points are eliminated or reduced: if applied to the wrong pairs of points, these forces have a large impact. 
\item \emph{Mesh dependence.} How these behave under remeshing or refinement: mesh adaptation, refinement, or remeshing are common, especially for large/complex deformations. 
\item \emph{Discretization properties.} If a potential is defined in continuous form, even if it prevents contact exactly, its discretization may do so only approximately. 
\end{itemize}

\paragraph{The IPC barrier potential \cite{Li2020IPC}}  This potential is defined in a purely discrete way, based on vertex-face and edge-edge repulsion.  To ensure it is \emph{finite}, interactions of a face with its vertices and between edges sharing one vertex are excluded.  \ZH{If we state this point as an issue of IPC, we need to be more careful about justifying that we ignore the adjacent pairs in the same way. Now the paragraph "Adjacent elements are excluded" in the \cref{sec:discretization} reads like we are just doing the same way as IPC.}

\begin{figure}
    \includegraphics[width=\linewidth]{figs/sketches/oipc-ipc-spurious-illustration.pdf}
    \caption{IPC potential.  The extent of the potential is shown in blue. 
    (1) IPC potential is finite, as interactions between edges sharing vertices, and faces with their vertices are dropped. (2) Refinement forces the maximal potential extent $\hat{d}$ to decrease. (3) Spurious forces (red arrows) arise if the surface is compressed horizontally and nearby vertices are closer than the potential extent $\hat{d}$.  
    }
    \label{fig:IPC-problems}
\end{figure}
    
\emph{Spurious forces} are partly avoided by defining a potential that does not extend beyond the shortest mesh edge length in the undeformed state.   However, during deformation, the edge length can change arbitrarily, and spurious forces may easily appear under compression.  
IPC potential is strongly \emph{mesh dependent}: e.g., simply refining locally forces the maximum extent of the potential to be decreased by a large factor, resulting in a change in the results of simulation/deformation. 

\paragraph{Surface/volume double-integral potentials \cite{sauer2013computational,Kamensky2018Contact}} Barrier potentials defined in continuum setting is used in \cite{Kamensky2018Contact}. 
To include self-contact, \emph{finiteness} is achieved by excluding a fixed-size area or sphere in the undeformed state from the integral. However, this exclusion eliminates the guarantee that under all deformations there is no penetration (Figure~\ref{fig:SL-problems}(1)).

To avoid \emph{spurious repulsion}, the potential is localized to a distance less than that of the self-contact exclusion distance (Figure~\ref{fig:SL-problems}(1)) In this way, in the undeformed state, there is no repulsion.  However, if compression is high enough, spurious forces will appear. 

To avoid \emph{spurious repulsion}, the potential is localized to a distance less than that of the self-contact exclusion distance. In this way, in the undeformed state, there is no repulsion.  However, if compression is high enough, spurious forces will appear (Figure~\ref{fig:SL-problems}(2)). 

As these potentials are defined as integrals on smooth surfaces and then discretized, there is a high degree of \emph{mesh independence}, especially for finer meshes, but may lead to self-intersection for sufficiently fine meshes or higher order elements as described above \MP{I'm a bit confused what precisely this is referring to. I don't think we've discussed higher order elements above}.  Furthermore, as pointed out in \cite{Kamensky2018Contact} the discretization based on pairwise potentials between quadrature points for extreme deformation may also result in failure to satisfy contact constraints. 

\begin{figure}
    \begin{center}
\includegraphics[width=\linewidth]{figs/sketches/surface-barrier-problems.png}
    \end{center}    
    \caption{Surface barrier of \cite{Kamensky2018Contact}. \MP{I can't find a description of self-contact/exclusion zones in the Sauer paper (the table agrees with this). I think this may mean to cite Kamensky.} (1) The potential has a self-contact exclusion zone (green), outside the potential extent (blue). For extreme deformations (folding), this allows self-intersections. (2) Extreme compression may push points into the potential zone, leading to spurious forces (arrow) (3) In quadrature point-to-point discretization, surface may not remain contact-free, a point may "push through" between other \protect\cite{Kamensky2018Contact}.
    }
    \label{fig:SL-problems}
\end{figure}

\paragraph{Repulsive shells \cite{repulsive2024}}  Building on, e.g. \cite{strzelecki2013tangent}, \cite{repulsive2024} introduced a repulsive potential, whose minimization can be used to define self-avoiding surfaces. 
An important feature of this potential in our context is that it handles the problem of near-point interactions gracefully for smooth surfaces, as the potential depends not only on positions but also on the normals. It vanishes in the limit of points approaching a common position on a smooth surface ensuring \emph{finiteness} for smooth surfaces, but not for surfaces with sharp features, as the normal alignment of close points is needed.  As these potentials are designed to ensure that surfaces minimizing these are $C^1$ (i.e., precisely to eliminate any possible sharp features), they use high inverse powers of distance, resulting in divergence for piecewise smooth surfaces.

 As the interaction potential for any curved surface does not vanish, \emph{spurious repulsion} is present for an undeformed surface (in the context of the target application of \cite{repulsive2024}, defining surfaces as extrema of the repulsive potentials, this repulsion is not spurious).  As the discretization used in \cite{repulsive2024} is based on sampling at quadrature point pairs similar to \cite{sauer2013computational}, it also does not guarantee in general that the contact constraints are satisfied exactly for the discretization, which is particularly important for coarse discretizations.   
 
 We further note that all these potentials depend smoothly on the surface deformation; the first two are local, and the last is global, although it decays rapidly. \ZH{"first two" and "last" are a bit ambiguous here.}

 \paragraph{Barriers based on the gap functions \cite{wriggers2006computational}}
    We briefly mention the possibility of constructing barriers based on gap functions, which can be viewed as solving a standard inequality-constrained contact problem formulation using an interior point method (e.g., \cite{kloosterman2001geometrical}, although this work shifts the barrier towards the interior of an object).

Most contact papers use one of three gap functions:  distance along the normal direction (DND), closest point (CP), and contact-pair closest distance (CPCD), the latter defined directly on discretization (e.g., vertex-face and edge-edge distances for PL surfaces).  \DZ{TODO: add citations from the appendix by type}
Most importantly, the CP gap function does not allow for self-contact, without explicit exclusion of nearby points, and while continuous, is not differentiable with respect to surface deformations (Figure~\ref{fig:gap-function-problems}(3)). 
The distance along the normal direction does resolve the self-interaction problem but is discontinuous hindering the application of efficient numerical methods (Figure~\ref{fig:gap-function-problems}(1)).   While the closest point distance is well-defined for distinct objects if they are not smooth, the distance along the normal direction requires a well-defined surface normal to exclude contact precisely. \ZH{I don't understand the previous sentence}


\begin{figure}
    \includegraphics[width=\linewidth]{figs/sketches/oipc-nonsmooth-gap.pdf}
\caption{(1) The NDD gap function is discontinuous when the deformation progresses from the black to the blue curve. (2) The NDD gap function can be arbitrarily small for p.w. smooth surfaces as $x_i$ approaches the sharp corner in a continuous setting. (3) The CP gap function changes non-smoothly, as the closest point switches discontinuously (from black to blue). }
\label{fig:gap-function-problems}
\end{figure}

A potential obtained by applying a logarithmic or inverse power function to these gap functions inherits the properties of these functions. 

Our construction addresses these problems by design, without the need for parameter tuning per simulation: for sufficiently close points, the potential vanishes exactly; no amount of compression leads to potential activation, unless surface points get close to contact; it is defined in a continuum form, so its behavior for different meshes is consistent; its strength is chosen so that it is sufficiently strong for smooth surfaces and does not blow up for piecewise smooth. Finally, we choose the discretization in a way that guarantees that the discretized surfaces are contact-free \ZH{exactly}. 


\section{Related Work}
\label{sec:related}


\DZ{TODO: make references consistent with the new supplementary material classification, penalty, augmented lagrangian,LCP/SQP}
Many methods for dynamic contact response formulate non-interpenetration constraints based on the normal displacements of the contacting regions with locally approximated geometries. Then the constrained time integration problem is solved with Lagrange multipliers~\cite{carpenter1991lagrange,deuflhard2008contact,hiermeier2018truly,Kane1999Finite,laursen2002improved,paoli2002numerical,paoli2002numerical2,taylor1993finite,vola1998consistent}, penalty methods~\cite{armero1998formulation,belytschko1991contact,hiermeier2018truly,hauret2006energy,Puso2004Mortar}, barrier methods~\cite{belytschko2000nonlinear,christensen1998formulation,kloosterman2001geometrical}, etc. To guarantee global convergence for the solution of frictionless large deformation contact problems for hyperelastic materials, \citet{youett2019globally} proposed a filter-trust-region method to solve the constrained minimization problem formulated from implicit time integration.

One common feature of all such methods,

Mortar methods~\cite{Belgacem1998Mortar,Hueber2006Mortar,Puso2004Mortar} are commonly used in engineering~\cite{Krause2016Parallel} and biomechanics~\cite{Maas2012FEBio} but require all possible pairs of contacting mesh boundaries to be marked a priori. \DZ{I do not think this is true for all mortar methods}

A clear limitation of these methods is that they cannot handle, without extensions, self-collisions or collisions in regions with more than two contacting surface regions. \citet{Li2020IPC} provide a didactic comparison of \ac{IPC} and one such mortar method~\cite{Krause2016Parallel}. There it can be seen that such methods enforce contact constraints weakly and therefore allow intersections (especially at large timesteps and/or velocities).

 \citet{sauer2013computational} formulate frictionless contact based on distance-dependent surface interaction potentials, providing a unified framework for various contact formulations including Lagrange multiplier, penalty, and barrier. 


\paragraph{Other barrier-based methods} %
In addition to the barrier methods based above,  most notably, \citet{Harmon2009Asynchronous} and \citet{Vouga2011Asynchronous} utilize a set of layered discrete penalty barriers that grow unbounded as the configuration approaches contact. However, this incremental construction makes it unsuitable for optimization-based implicit time integration and therefore requires small time-steps for stability.

\citet{Kaldor2008Simulating} simulate knitted cloth at the yarn level 
where yarn-yarn collisions are handled through a continuous potential integrating a barrier function over two disjoint spline segments. This approach, similarly to surface potentials described above,  ignores self-collisions within a single segment and between neighboring segments. Similarly, this work uses quadrature points fixed in the parameter space to compute interactions, which may introducing intersections.


The method of \citet{Li2020IPC} has been directly utilized and extended by numerous follow-up works to include support for codimensional elements~\cite{Li2021Codimensional}, rigid/affine body dynamics~\cite{Ferguson2021Intersection,Lan2022Affine}, medial elastics~\cite{Lan2021Medial}, solid-fluid interactions~\cite{xie2023contact}, higher-order finite element analysis~\cite{Ferguson2023HighOrderIPC}, etc.

The most significant limitation of \ac{IPC}~\cite{Li2020IPC} is its lack of convergence under mesh refinement due to its purely discrete formulation (see \citet{Li2023Convergent} for details). 
To address this, \citet{Li2023Convergent} form a continuous formulation for the original \ac{IPC} model which requires minimal adjustments to existing implementations. Limitations of their approach include (a) the requirement for joint refinement of $\dhat$ and mesh resolution (b) the lack of considering normal and tangent directions. Our method decouples the choice of $\dhat$ and mesh resolution, providing more flexibility in choices of parameters, which is useful to accelerate convergence and simulate on adaptive meshes. By considering normal and tangent directions of the surface, our method resolves artifacts that are not handled by \citet{Li2023Convergent}. We provide further discussion and comparisons in \cref{sec:eval} and \cref{tab:compare_other}.

\begin{table*}[htb]
    \centering
    \small
    \begin{tabular}{c|c|c|c|c|c|c}
         & Self-contact & Intersection-free & Convergence & Resolution independence & Surface normals \\ \hline
         \citet{Li2020IPC} & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes & \cellcolor{red!25}No & \cellcolor{red!25}No & \cellcolor{red!25}No \\
         \citet{Li2023Convergent} & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes & \cellcolor{red!25}No & \cellcolor{red!25}No \\
         \citet{Larionov2021Frictional} & \cellcolor{red!25}No & \cellcolor{red!25}No & \cellcolor{red!25}No & \cellcolor{red!25}No & \cellcolor{green!25}Yes\\
         \citet{Du2023Free} & \cellcolor{green!25}Yes & \cellcolor{red!25}No & \cellcolor{red!25}No & \cellcolor{red!25}No & \cellcolor{green!25}Yes\\
         Ours & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes & \cellcolor{green!25}Yes\\
    \end{tabular}

    \caption{The table columns correspond to six comparison characteristics: (1) Support self-contact, (2) guarantee intersection-free with conservative CCD, (3) the contact potential converges under mesh refinement, (4) the support size of contact barrier, i.e. $\dhat$, can be independent of mesh resolution, (5) can filter undesired contact based on surface normals. We refer to \cref{sec:related} and \cref{sec:eval} for detailed discussions.} %
    \label{tab:compare_other}
\end{table*}

\ZH{Modified below because now they have "self-contact".}
\DZ{TODO: this is way too detailed}
\citet{Du2023Free} shows the tendency of ``Node-to-Segment'' methods (e.g., IPC~\cite{Li2020IPC}) to produce spurious tangential contact forces. 
 We do not aim to address this type of artifact in our discretization -- our work is complementary, although a higher-order discretization of our potential may be suitable for this. \citet{Du2023Free}  proposes to use a fully $C^1$-continuous surface representation, computing distances used in the contact potential between the nodes and smooth surface (extending the method of \citet{Larionov2021Frictional}). The main limitation of \citet{Du2023Free} and \citet{Larionov2021Frictional}, however, is a lack of robust handling self-collisions and the absence of conservative CCD (Table~\ref{tab:compare_other}),  features critical for IPC's robustness~\cite{Li2020IPC}. \citet{Du2023Free} supports self-collision by ignoring the collision of a vertex with its geodesic neighborhood, with a user-specified parameter to control the size of the neighborhood, leading to the possibility of local intersection. Besides, subdivisions are needed to approximate the original sharp object with the smooth representation, resulting in a much higher cost in each Newton iteration compared with \citet{Li2020IPC}.

\ZH{Contact papers at Siggraph2024}
Recently, \citet{HUANG2024GIPC} proposes using a matrix-free preconditioned conjugate gradient solver that is amenable to GPU data parallelism to accelerate \cite{Li2020IPC}. Similarly, \citet{Shen2024PreconditionedIPC} proposes a preconditioned nonlinear conjugate gradient method that runs on GPU, enabling real-time simulation of objects comprising over 100K tetrahedra. However, it replaces the \ac{CCD} with a non-robust check inspired by the CFL condition, leading to penetration or failure of convergence in some challenging cases like mat-twisting as pointed out in the paper.

\DZ{rewrite}
\paragraph{Tangent-point energies}
A possible continuous approach to avoiding intersections is the tangent-point energies~\cite{buck1995simple,strzelecki2013tangent}. We follow the notations in \cite{Yu2021RepulsiveSurfaces}: Given a surface $M$ and an immersion $f: M \rightarrow \mathbb{R}^3$, the tangent-point energy repels displaced surface points by integrating over all surface pairs $(x,y) \in M\times M$:
\begin{equation}\label{eq:repulsive_original}
    \mathcal{E}(f):=\iint_{M\times M} \frac{\|P_f(x)(f(x) - f(y))\|^p}{\|f(x)-f(y)\|^{2p}}~\mathrm{d}x_f\mathrm{d}y_f,
\end{equation}
where $\mathrm{d}x_f$ denotes the area element induced by $f$, $p=6$ controls the repulsion strength, and $P_f(x)=N_f(x)N_f(x)^\top$ denotes the orthogonal projector onto the normal $N_f(x)$ at $x$. 

Recently, \citet{Yu2021RepulsiveCurves,Yu2021RepulsiveSurfaces,Sassen:2024:RS} utilize tangent-point energies to prohibit intersections while optimizing surface geometry. In pure form, this method works well in the context of smooth surface optimization but is unsuitable for collision response due to its global coupling of all points. It is related to our approach as discussed in Section~\ref{sec:contact-candidates} in the case of smooth surfaces. It also does not fully prevent spurious local repulsion, if applied in simulation contexts, and these energies are infinite for surfaces with sharp features (\cref{sec:repulsive}). For piecewise linear meshes, the normals are not unique at vertices, to avoid this issue, \cite{Yu2021RepulsiveSurfaces,Sassen:2024:RS} use a single-point quadrature rule at face centers (where the normals are unique), with the sacrifice that edges may intersect even though faces are penetration-free. 



==> 41-pw-smooth-construction-old.tex <==

\subsection{Piecewise smooth contact}\label{sec:pw-sm}
 We now extend the potential to piecewise smooth surfaces. There are two reasons for this extension: (1) piecewise smooth surfaces are ubiquitous in graphics and scientific computing as they can represent shapes with sharp features, and (2) smooth surfaces are often approximated by piecewise linear for which efficient robust continuous collision detection is available.


We consider surfaces consisting of patches $\boundary_i$, which form a possibly curved manifold mesh satisfying the standard definition \cite{do2016differential}. We assume that each patch has continuously varying normals defined everywhere including boundary (i.e. no cones are allowed) the edge curves meeting at a vertex, and faces meeting at an edge have distinct tangents and tangent planes in the undeformed shape. We refer to the curves separating patches as \emph{edge curves}, or simply edges, and points shared by more than two patches
as vertices.


In this case, there are six possibilities for a contact point, corresponding to the possible pairs of contacts between any two element types: Face-Face, Face-Edge, Face-Vertex, Edge-Edge, Edge-Vertex, Vertex-Vertex. We handle all these cases together in a uniform way.


\subsubsection{\textbf{{\Interaction} sets for piecewise smooth surfaces}}
We use the same general definition for {\interaction} sets $C(x,f)$ for piecewise smooth surfaces. Specifically, \emph{$C(x,f)$ is the set of points $y$ close in the sense defined below to local minima of the distance function $\|f(y)-f(x)\|$, and with the vector $f(y)-f(x)$ pointing to the exterior of the surface at $x$ and to the interior at $y$}. 

However, more complex machinery is needed to convert this to a mathematical definition compared to $\Phi^m$ and $\Phi^e$ functions for smooth surfaces.  Most of the effort required is to express the simple definition above as smooth functions of $f$. 

\paragraph{Local minimum constraint}
Consider the distance $\|f(y) - f(x)\|$ as a function of $y$. If the closest point is in the interior of some patch $\Omega_i$, i.e. the contact point is a face point, then for the gradient w.r.t. $y$, we obtain
\begin{equation}\label{eq:minima}
    \transpose{\nabla_y f(y)}~(f(y)-f(x))_+ = 0
\end{equation}
at the closest point, where the gradient $\nabla_y$ is computed with respect to a parametrization of $\boundary_i$. The columns of the matrix $\nabla_y f$ are two tangents at $y$, i.e., this condition is equivalent to the condition that $n(y)$ is parallel to $f(y)-f(x)$ in the definition of $C(x,f)$.

To generalize the minimum condition to edge and vertex contact points on piecewise smooth surfaces, consider the set of patches $\boundary_i$ containing a point $y$ (one patch for face points, two for edge points, and any number for vertex points). For each $\boundary_i$ and each parametric direction $p\in\mathbb{R}^2$ at $y$, there is a well-defined unit tangent direction $t:=\partial_p f(y)$ of $\boundary_i$. The directional derivative $\partial_p $ is one-sided if $y$ is on the boundary of $\boundary_i$.

The condition for a local minimum is that for any $\boundary_i$, the distance does not decrease along any tangent $t$, i.e.,
\begin{equation}\label{eq:parametric_minima}
    \transpose{t}~(f(y)-f(x))_+  \geq  0
\end{equation}

If $y$ is on more than one patch, i.e. on the shared boundary of patches, on each patch $\boundary_i$, there are two tangent vectors $t^1_i(y)$ and $t^2_i(y)$, along two edge curves of $\boundary_i$ meeting at $y$ (\cref{fig:tangent-notation}). If $\transpose{t^j_i(y)}~(f(y)-f(x))_+\geq 0$, then for any $t=\sum_{j=1}^2 a_j t^j_i(y)~(a_j\geq 0)$, we have
$$
\transpose{t}~(f(y)-f(x))_+ = \sum_{j=1}^2 a_j \transpose{t^j_i(y)}~(f(y)-f(x))_+\geq 0,
$$
which means \cref{eq:parametric_minima} holds for any $t$ in the convex cone spanned by $t^1_i(y)$ and $t^2_i(y)$ (\cref{fig:tangent-notation} A). However, the tangent directions of $\Omega_i$ at $y$ may not always lie in the cone. For example, when $y$ is on an edge of a linear triangle as $\boundary_i$, $t^1_i(y) + t^2_i(y) = 0$, then the convex cone degenerates to a line, while the tangent directions form a half-plane (\cref{fig:tangent-notation} B); when $y$ is at a concave corner of a high order patch $\boundary_i$, then the convex cone is the complement of $\boundary_i$ (\cref{fig:tangent-notation} C).


To treat all cases uniformly, we add a halfway vector $t^3_i$, corresponding to the angle bisector of the angle between $t^1_i$ and $t^2_i$ in $\boundary_i$ (\cref{fig:tangent-notation}). Then every tangent vector $t$ of $\Omega_i$ at $y$ can be represented as a convex combination of $\{t^j_i\}_{j=1}^3$, and consequently, \cref{eq:parametric_minima} along these three directions ensures that the point is a local minimum of the distance.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/sketches/tangent-notation.pdf}
    \caption{Notation for tangents in \cref{def:contactmin} in 3D. $\boundary_i$ is a face (not necessarily triangle) in 3D colored with light purple, $t_1$ and $t_2$ are the two tangent vectors at $f(y)$, $t_3$ is the angle bisector of the angle between $t_1$ and $t_2$. The face is viewed from the normal direction. 
    }
    \label{fig:tangent-notation}
\end{figure}




\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/cone-filter/cone-filter.pdf}
    \caption{Problem setup of determining if a vector $v$ (red) is pointing inside of the piecewise linear surface. Point $f(y)$ and its 1-ring neighbors on the piecewise linear surface (gray) intersect with a small sphere (green) centered at $f(y)$, their intersection is shown in blue. The intersection in 3D is not necessarily convex (middle).%
    }
    \label{fig:cone-filter-setup}
\end{figure}

\paragraph{Exterior direction constraint}
The analog of $\Phi^e(x,y)>0$ requires a criterion for determining that a unit vector $v:=(f(y) - f(x))_+$ at a point $f(y)$ of a closed piecewise smooth surface points inside. For piecewise linear surfaces, as in \cref{fig:cone-filter-setup}, the point $f(y)$ and its 1-ring neighbors form a cone.  Consider a small sphere centered at $f(y)$, its surface is partitioned into two parts by the cone and $v$ intersects the sphere surface at one point. The problem is identifying the part of the sphere containing the point. 
For high-order surfaces, determining if $v$ points inside only requires checking the cone formed by the tangent planes at $f(y)$, which is equivalent to considering the same problem for piecewise linear surfaces.

We are going to define a function $\Phi^e(x, y)$ that is positive if and only if $v$ points inwards at $f(y)$.  Consider the problem in 2D (\cref{fig:cone-filter-setup}). The two incident edges at $f(y)$ are $e_1,\ e_2$, with corresponding normals $n_1,\ n_2$. We assume all vectors have unit length since we only care about the directions. Suppose $e_1\times n_1>0$ (otherwise swap $e_1$ and $e_2$), to determine if $v$ points outside the surface we only need to check if $e_1,\ v,\ e_2$ are in counter-clockwise order, so we can define
\begin{equation}\label{eq:cone-filter-2D}
    \Phi^e(x, y):=(v-e_1)\times(v-e_2).
\end{equation}
Note that $\Phi^e(x,y)=0$ if and only if $v,\ e_1,\ e_2$ are on the same line, i.e. $v$ overlaps with $e_1$ or $e_2$.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/cone-filter/cone-filter-algo-2.pdf}
    \caption{3D (left) and 2D (right) views of the closest point on an edge. The 2D view is the projection of the 3D view onto the plane perpendicular to the edge $e_j$. $\tilde{v}, \tilde{e}_1, \tilde{e}_2$ are the projections of $v, e_{j-1}, e_{j+1}$ respectively. $\tilde{n}_1$ is the projected normal of the face bounded by $e_{j-1},e_j$. Deciding if $v$ points inside the cone in 3D is equivalent to deciding if $\tilde{v}$ is inside the sector bounded by $\tilde{e}_1$ and $\tilde{e}_2$ in 2D.}
    \label{fig:closest-shared}
\end{figure}

In 3D, we first discuss $\Phi^e(x,y)$ for edges in Edge-Vertex and Edge-Edge contact. As shown in \cref{fig:closest-shared}, to determine if a vector $v$ points inwards, we can project everything onto the plane perpendicular to edge $e_j$ and apply \cref{eq:cone-filter-2D} on the projected vectors. For vertices, however, defining $\Phi^e(x,y)$ becomes more complicated. A detailed description of how to define $\Phi^e(x,y)$ in a robust fashion for vertices is included in \cref{app:outside-filtering}. This leads to the following definition of a {\interaction} set:

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/sketches/normal-demo.pdf}
    \caption{2D (top) and 3D (bottom) normal directions for contact points. $f(y) - f(x)$ is shown in yellow; $n_i(y)$ are shown in red if \cref{eq:normal} is satisfied, otherwise green. Tangent directions are shown in blue in 3D. In simple contact cases, e.g. (A) and (D), the normals all satisfy \cref{eq:normal}, but in other cases, not all normals satisfy the inequality.}
    \label{fig:normal-notation}
\end{figure}

\begin{definition}[{\Interaction} sets for p.w. smooth surfaces]
For each point $y$ of $\boundary$, let $I$ be the set of indices of patches $\boundary_i$ containing $y$, and  for each patch, define $t^k_i(y)$, $k=1,2,3$ as above.  Then $C(x,f)$ consists of points $y$ satisfying
\begin{equation}
\begin{split}
&\Phi^m_{ik}(x,y):= \transpose{t^k_i(y)} (f(y)-f(x))_+  \geq -\alpha,\\
&\Phi^m_{ik}(y, x) \geq -\alpha,\;
\Phi^e(x,y) \geq -\beta,\;
\Phi^e(y, x)  \geq -\beta,\;
\end{split}
\label{eq:pw-contact-alpha}
\end{equation}
for $i \in I$, $k=1,2,3$, $0<\alpha\leq 1$, and $0<\beta\leq 1$ is a separate parameter that controls the smoothness of $\Phi^e$. We use $\beta=0.1$; the specific choice of $\beta$ has little impact on the method's behavior and numerical stability. 
\label{def:contactmin}
\end{definition}

\begin{remark}

The size of the index set $I$ depends on the type of primitive being considered: In 2D, edge curves have size $|I|=1$; vertices have $|I|=2$, including the two edges joined at this vertex. In 3D, faces have $|I|=1$, edge curves have $|I|=2$, and vertices have $|I|\geq 2$.
\end{remark}


\ZH{Try to move the following to the appendix}

\subsubsection{\textbf{\Smoothingfactor}} 

\paragraph{Local minimum term} The mollification of local minimum constraints $\Phi^m_{ik}(x,y)\geq -\alpha,\ \forall i\in I$ is straightforward and similar to the smooth surface case:
$$
g^m(x,y):=\prod_{i\in I}\prod_{k=1}^{3} H^{\alpha}(\Phi^m_{ik}(x,y))
$$
reaches maximum of 1 when $\Phi^m_{ik}(x,y)\geq 0,\ \forall i\in I$, and vanishes if there exists $i\in I$ such that $\Phi^m_{ik}(x,y)\leq -\alpha$.

Since $\Phi^m_{ik}$ is a dot product between unit vectors, $\alpha$ acts as a threshold of contact potential on the cosine value of the angle between contact pairs. One can pick $\alpha$ based on the desired angle threshold, we use $0.05\leq \alpha\leq 0.8$ in the examples. Although extremely small $\alpha$ leads to numerical issues in the simulation, \cref{req:barrier} is satisfied as long as $\alpha>0$, i.e. the simulation is always contact-free.

\paragraph{Exterior direction term} For edge points in Edge-Edge and Edge-Vertex contact, based on \cref{eq:cone-filter-2D} we can define 
$$
g^e(x,y) := H^\beta (\Phi^e(x,y)),
$$
where $\beta$ is a parameter that controls the smoothness of exterior direction constraints. $g^e(x,y)$ reaches maximum when $\Phi^e(x,y)\geq 0$ and vanishes if $\Phi^e(x,y)\leq -\beta$. 

For vertices in Face-Vertex, Edge-Vertex, and Vertex-Vertex contact, we first define 
$$
\Phi^e_{i}(x,y):=-\transpose{n_i(y)} (f(y)-f(x))_+.
$$
However, unlike the case of the smooth surfaces, there are multiple normal directions at one vertex (\cref{fig:normal-notation}). To eliminate the contact between opposite sides of the object (Figure~\ref{fig:candidates}), the following should hold for some $i\in I$
\begin{equation}\label{eq:normal}
    \Phi^e_{i}(x,y) \geq 0 .
\end{equation}
To make the constraint smooth, we relax this to a simpler, weaker condition. We define 
\begin{equation}\label{eq:normal_mollified}
g^e(x,y) :=H^{1}\left(-1+\sum_{i\in I} H^{\beta}\left(\Phi^e_{i}(x,y)\right)\right),
\end{equation}
which reaches a maximum of 1 when there exists $i$ such that
$
\Phi_{i}^e(x,y) \geq 0,
$
and vanishes if for all $i$,
$
\Phi_i^e(x,y) \leq -\beta.
$ 

\subsubsection{\textbf{Contact potential for piecewise smooth surfaces}}  Using the new definition of {\interaction} sets $C(x)$ and combining the local minimum and exterior direction constraints, we get, similar to the smooth case, 
\begin{equation}\label{eq:pw-angle-factor}
\begin{split}
&g^{PS}(x,y) := g^e(x,y) g^m(x,y)\\
&\gamma^{PS}(x,y) := g^{PS}(x,y) g^{PS}(y,x)
\end{split}
\end{equation}

However, one cannot simply replace $\gamma^{S}(x,y)$ with $\gamma^{PS}(x,y)$ in \cref{eq:potential-deform} to obtain the potential for the piecewise smooth case.  Recall that contact may happen to measure-zero sets on the piecewise smooth surface, e.g. vertex-vertex and edge-edge contact. As a consequence, the contact set in these configurations has zero measure (edge curves and vertices in 3D), and direct surface integration of $\psi(x)$ will lead to a zero potential.

For this reason, we treat low-dimensional elements separately. Informally, we can think about the interaction of lower-dimensional elements, as expanding them into areas: e.g., an area of width $L$ along curves, and an area of size $L^2$ assigned to vertices, with the potential constant along the direction in the area orthogonal to the curve, or on the whole area assigned to a vertex.  More precisely, this corresponds to adding line integrals for edge curves weighted by $L$, and points sums for vertices, weighted by $L^2$.  The potentials we integrate for a pair of elements $G$ and $H$, possibly of different dimensions, e.g., with $G$ being a vertex and $H$ a face,  can be written in the form
\[
P(x,y; G, H) = \gamma^{PS}(x,y; G, H)\pe(x,y)
\]
where $\gamma^{PS}(x,y; G, H)$ is the factor defined in \cref{eq:pw-angle-factor}, \emph{for $x$ considered as a point on element $G$,} in other words, if $G$ is a face, and $x$ happens to be an edge or vertex point, the factor $\gamma^{PS}(x,y)$ is computed using formulas for face points $x$. 


Then the total potential can be written as
\begin{equation}\label{eq:pwpot}
\Psi(f) = \sum_{ (g,h) } \sum_{\substack{i \in I_g, j \in I_h\\ G_i \cap H_j = \varnothing}} L^{4-\dim g - \dim h} \int_{G_i}\int_{H_j} P(x,y; G_i, H_j)~\mathrm{d}x\mathrm{d}y
\end{equation}
where $g,h$ are one of the element types $\{\text{Face}, \text{Edge}, \text{Vertex}\}$, with the first sum is over 9 unordered pairs, $I_g$ and $I_h$ are sets of indices of elements of types $g$ and $h$, and $G$ and $H$ element indices.  The integrals are area, line, or 0-dimensional, i.e. simple evaluations for vertices. %


\begin{prop}
The potential  \eqref{eq:pwpot} satisfies \cref{req:barrier,req:no-spurious-forces,req:localization,req:differentiability,req:generality} if $f$ is piecewise-curvature-continuous surface as defined in this section, with $C(x,f)$ given by \cref{def:contactmin},  distance-to-contact defined as 
$d_c(x,f) := \min_{y\in C(x,f)} \| f(y) - f(x)\|$, and $\gamma(x,y)$ given by \cref{eq:pw-angle-factor}.
\label{prop:pwsmooth-properties} 
\end{prop}
Please see the supplementary document for details. 


\paragraph{Parameters of the potential} Whether the potential satisfies contact potential requirements does not depend on the choice of $L > 0$, $\epsilon_\text{trg} > 0$,
and $0 < \alpha < 1$, as long as these are positive. There is no strong impact on robustness, as long as the values are not too close to the bounds,
but may affect performance. 

\begin{itemize}
    \item $\alpha$ determines the size of the {\interaction} sets, and as a consequence how smoothly the potential depends on $f$. The closer $\alpha$ is to zero, the less smooth the dependence is, but the more localized it is.
    \item $\epsilon_{trg}$ determines the upper bound on how far the potential extends ($\hat{d}$ in IPC) but especially at concave corners, $\epsilon_{trg}$ as well as $f_0$, affect this.
    \item $L$ %
    determines the strength of potential for low-dimensional contact. In our examples, for vertices, we set it to the average edge length around the vertex; for edges, we set it to the length of the edge; for faces, $L$ is not needed.
   
\end{itemize}



==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}


